A Wolf in Sheep's Clothing: Generalized Nested Jailbreak Prompts can Fool Large Language Models Easily

Large Language Models (LLMs), such as ChatGPT and GPT-4, are designed to provide useful and safe responses. However, adversarial prompts known as 'jailbreaks' can circumvent safeguards, leading LLMs to generate potentially harmful content. Exploring jailbreak prompts can help to better reveal the weaknesses of LLMs and further steer us to secure them. Unfortunately, existing jailbreak methods either suffer from intricate manual design or require optimization on other white-box models, which compromises either generalization or efficiency. In this paper, we generalize jailbreak prompt attacks into two aspects: (1) Prompt Rewriting and (2) Scenario Nesting. Based on this, we propose ReNeLLM, an automatic framework that leverages LLMs themselves to generate effective jailbreak prompts. Extensive experiments demonstrate that ReNeLLM significantly improves the attack success rate while greatly reducing the time cost compared to existing baselines. Our study also reveals the inadequacy of current defense methods in safeguarding LLMs. Finally, we analyze the failure of LLMs defense from the perspective of prompt execution priority, and propose corresponding defense strategies. We hope that our research can catalyze both the academic community and LLMs developers towards the provision of safer and more regulated LLMs. The code is available at https://github.com/NJUNLP/ReNeLLM.

==> 1_Introduction.tex <==
\section{Introduction}

The emergence of Large Language Models (LLMs) has played a pivotal role in driving the advancement of Artificial Intelligence (AI) systems. Noteworthy LLMs like ChatGPT \citep{OpenAI, OpenAI-4}, Claude2 \citep{Claude2}, Bard \citep{Google}, and Llama2 \citep{touvron2023llama} have demonstrated their advanced capability to perform innovative applications, ranging from tool utilization, supplementing human evaluations, to stimulating human interactive behaviors \citep{jiao2023chatgpt,bubeck2023sparks, schick2023toolformer, DBLP:conf/acl/ChiangL23, park2023generative}.
The outstanding competencies have fueled their widespread deployment, while the progression is shadowed by a significant challenge: {\em ensuring the safety and reliability of the responses}.

To harden LLMs for safety, there has been a great body of work for aligning LLMs with human ethics and preferences to ensure their responsible and effective deployment, including data filtering \citep{xu2020recipes,welbl-etal-2021-challenges-detoxifying, wang2022exploring}, supervised fine-tuning \citep{ouyang2022training}, reinforcement learning from human feedback (RLHF) \citep{christiano2017deep}, and red teaming \citep{perez2022red, ganguli2022red, OpenAI-4}. 
The majority of existing work on safety alignment has focused on the inputs and outputs in {\bf natural languages}. 
However, recent works show that LLMs exhibit unexpected capabilities in understanding {\bf non-natural languages} like the \texttt{Morse Code} \citep{morse_jail}, \texttt{ROT13}, and \texttt{Base64} \citep{wei2023jailbroken}.
One research question naturally arises: {\em can the non-natural language prompt bypass the safety alignment mainly in natural language?}

To answer this question, we propose a novel framework {\em CipherChat} to systematically examine the generalizability of safety alignment in LLMs to non-natural languages -- ciphers.
CipherChat leverages a carefully designed system prompt that consists of three essential parts: 
\begin{itemize}[leftmargin=10pt]
    \item {\em Behavior assigning} that assigns the LLM the role of a cipher expert (e.g. ``{\em You are an expert on \texttt{Caesar}}''), and explicitly requires LLM to chat in ciphers (e.g. ``{\em We will communicate in \texttt{Caesar}}'').
    \item {\em Cipher teaching} that teaches LLM how the cipher works with the explanation of this cipher, by leveraging the impressive capability of LLMs to learn effectively in context.
    \item {\em Unsafe demonstrations} that are encrypted in the cipher, which can both strengthen the LLMs' understanding of the cipher and instruct LLMs to respond from a negative perspective.
\end{itemize}
CipherChat converts the input into the corresponding cipher and attaches the above prompt to the input before feeding it to the LLMs to be examined. LLMs generate the outputs that are most likely also encrypted in the cipher, which are deciphered with a rule-based decrypter.

We validate the effectiveness of CipherChat by conducting comprehensive experiments with SOTA \texttt{GPT-3.5-Turbo-0613} (i.e. Turbo) and \texttt{GPT-4-0613} (i.e. GPT-4) on 11 distinct domains of unsafe data~\citep{sun2023safety} in both Chinese and English.
Experimental results show that certain human ciphers (e.g. \texttt{Unicode} for Chinese and \texttt{ASCII} for English) successfully bypass the safety alignment of Turbo and GPT-4. 
Generally, the more powerful the model, the unsafer the response with ciphers.
For example, the \texttt{ASCII} for English query succeeds almost 100\% of the time to bypass the safety alignment of GPT-4 in several domains (e.g. {\em Insult} and {\em Mental Health}). The best English cipher \texttt{ASCII} achieves averaged success rates of 23.7\% and 72.1\% to bypass the safety alignment of Turbo and GPT-4, and the rates of the best Chinese cipher \texttt{Unicode} are 17.4\% (Turbo) and 45.2\% (GPT-4).


A recent study shows that language models (e.g. ALBERT \citep{Lan2020ALBERT:} and Roberta \citep{liu2019roberta}) have a ``secret language'' that allows them to interpret absurd inputs as meaningful concepts \citep{wang2023investigating}. Inspired by this finding, we hypothesize that LLMs may also have a ``secret cipher''. Starting from this intuition, we propose a novel \texttt{SelfCipher} that uses only role play and several demonstrations in natural language to evoke this capability, which consistently outperforms existing human ciphers across models, languages, and safety domains.



% \paragraph{Contributions}
Our main contributions are:
\begin{itemize}[leftmargin=15pt]
    \item Our study demonstrates the necessity of developing safety alignment for non-natural languages (e.g. ciphers) to match the capability of the underlying LLMs.

    \item We propose a general framework to evaluate the safety of LLMs on responding cipher queries, where one can freely define the cipher functions, system prompts, and the underlying LLMs.

    \item We reveal that LLMs seem to have a ``secret cipher'', based on which we propose a novel and effective framework \texttt{SelfCipher} to evoke this capability.

\end{itemize}


